PhiShark2026: A Multi-Layer Active-Web Raw-Evidence Dataset for Phishing Website Research

Phishing websites are short-lived and rapidly changing, yet many phishing datasets reduce observations to URLs or precomputed features, constraining researchers to predefined representations and discarding the underlying evidence needed to derive alternative features, apply new extraction methods, examine cross-layer relationships, and reanalyze observations as phishing techniques evolve. This study addresses this limitation with a multi-layer active-web dataset comprising 67,502 scans, including 33,387 phishing observations from operational feeds and 34,115 screened benign reference observations. The corpus preserves raw evidence across HTML content and screenshots, URL and redirect behavior, HTTP and security headers, compliance files, TLS certificates, DNS and domain registration, open ports, geolocation and accessibility measurements, and network infrastructure, while explicitly recording unavailable evidence rather than treating it as negative observations. To avoid misleading infrastructure attribution on shared platforms, the study applies a hosting-aware evidence model that masks provider-owned infrastructure signals for free-hosted tenant pages while retaining meaningful page- and transport-level evidence. Characterization reveals systematic differences between phishing and benign websites across web-resource usage, domain maturity, mail and policy configuration, security headers, and infrastructure context. By preserving raw artifacts together with acquisition metadata and explicit evidence availability, the corpus provides an inspectable and reproducible foundation for future phishing measurement and dataset research.

==> sections/proposed-dataset.tex <==
\label{proposed-dataset}

\newcommand{\collectionarchitecturefigure}{%
\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{figures/data-collection.png}
  \caption{Distributed active-web acquisition architecture used to build the corpus. Submitted targets are canonicalized, routed to parallel specialized fetchers, and persisted under a shared scan identifier.}
  \label{fig:data-collection-flow}
\end{figure*}%
}

\newcommand{\sourceaccountingtable}{%
\begin{table*}[!t]
  \centering
  \caption{Source provenance, collection intervals, and complete class-by-hosting distribution.}
  \label{tab:source-accounting}
  \footnotesize
  \setlength{\tabcolsep}{4.2pt}
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}Xlrrr>{\raggedright\arraybackslash}p{3.5cm}}
    \toprule
    \textbf{Source or summary} & \textbf{Class} & \textbf{Free host} & \textbf{Non-free} & \textbf{Total} & \textbf{Collection interval (UTC)} \\
    \midrule
    OpenPhish~\cite{openphishfeeds2026} & Phishing & 14,633 & 16,245 & 30,878 & 2026-04-23 to 2026-08-15 (113.9 days) \\
    Malicious Links List (Cybersecurity Presidency)~\cite{sgb2026maliciouslinks} & Phishing & 453 & 2,056 & 2,509 & 2026-06-14 to 2026-08-15 (62.1 days) \\
    OpenPageRank~\cite{openpagerank2026top} & Benign & 15,359 & 18,756 & 34,115 & Targeted snapshots \\
    \midrule
    \multicolumn{6}{l}{\textit{Class and corpus totals}} \\
    Phishing total & Phishing & 15,086 & 18,301 & 33,387 & \\
    Benign total & Benign & 15,359 & 18,756 & 34,115 & \\
    \textbf{Overall total} & \textbf{All} & \textbf{30,445} & \textbf{37,057} & \textbf{67,502} & \\
    \bottomrule
  \end{tabularx}
\end{table*}%
}

This collection is an active-web phishing corpus intended for controlled research access and designed around artifact preservation rather than a fixed derived table. Its unit of observation is a scan: a target URL acquired at a specific point in time together with the page, transport, registration, and infrastructure evidence successfully observed during that acquisition. This design allows approved researchers to audit collection failures, construct alternative representations, and revisit analytical assumptions, consistent with calls for transparent dataset documentation and more complete phishing-resource collection \cite{gebru2021datasheets,kulkarni2025collector}.

\section{Data Sources}

Phishing targets are drawn from two operational sources: OpenPhish and the Malicious Links List, maintained by the Cybersecurity Presidency of the Republic of Türkiye \cite{openphishfeeds2026,sgb2026maliciouslinks}. These feeds provide operationally reported targets rather than a complete census of phishing activity; source-specific collection intervals are reported with the dataset composition in Section~\ref{sec:dataset-composition-availability}.

\ifanonsubmission\else
  \collectionarchitecturefigure
\fi

\section{Acquisition Architecture}

Each target is canonicalized into URL-, host-, and registrable-domain forms before a distributed acquisition pipeline dispatches browser, network, DNS, TLS, WHOIS/RDAP, geolocation, compliance-path, and port-observation workers. Browser and network tasks run through a consistent collection policy with proxy-backed retrieval to reduce region-specific blocking and transient crawl gaps. All outputs are joined by a shared scan identifier. Figure~\ref{fig:data-collection-flow} summarizes this routing and acquisition path.

\ifanonsubmission
  \collectionarchitecturefigure
\fi

The acquisition pipeline routes the canonical full URL, full host, or registrable domain to eight specialized fetchers. Table~\ref{tab:fetcher-implementations} records the acquisition mechanism and retained evidence for each fetcher.

\begin{table}[!t]
  \centering
  \caption{Fetcher implementations and preserved evidence.}
  \label{tab:fetcher-implementations}
  \scriptsize
  \setlength{\tabcolsep}{2.8pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{1.22cm}>{\raggedright\arraybackslash}p{2.45cm}>{\raggedright\arraybackslash}X}
    \toprule
    \textbf{Fetcher} & \textbf{Input and mechanism} & \textbf{Preserved evidence} \\
    \midrule
    Web & Full URL; headless Chromium through \texttt{chromedp} and the Chrome DevTools Protocol \cite{chromedp2026} & Rendered HTML, screenshot, redirects, outgoing links, detected technologies, and browser/network statistics \\
    DNS & Registrable domain; \texttt{miekg/dns} with the Go resolver as fallback \cite{miekgdns2026} & A, AAAA, MX, NS, TXT, CNAME, and SOA records \\
    TLS & Full host; Go \texttt{crypto/tls} and \texttt{crypto/x509} & Issuer, subject, validity, serial number, SANs, and negotiated TLS version \\
    Domain registration & Registrable domain; RDAP client and registry bootstrap \cite{hollenbeck2021rdap} & Registrar, registration dates, nameservers, registrant country, DNSSEC, and raw response \\
    Compliance & Full host; bounded HTTP retrieval of public well-known paths & Locations of \texttt{security.txt}, \texttt{robots.txt}, \texttt{sitemap.xml}, and related public files \cite{foudil2022rfc9116} \\
    IP geolocation & Resolved IP; IP-API JSON endpoint \cite{ipapi2026} & Country, region, city, coordinates, timezone, ISP, organization, and AS \\
    IP WHOIS & Resolved IP; WHOIS client and parser \cite{likexianwhois2026} & Network range, CIDR, organization, country, ASN/origin, abuse contact, and registration dates \\
    Port observation & Resolved IPv4; ProjectDiscovery Naabu top-100-port profile \cite{projectdiscoverynaabu2026} & Resolved address, observed open ports, and scan duration \\
    \bottomrule
  \end{tabularx}
\end{table}

\section{Benign Reference Construction}

The benign candidate pool was sampled at random from the OpenPageRank Top 10 Million Domains list, whose domain-level authority ranking is derived from the Common Crawl web graph \cite{openpagerank2026top}. Independently registered candidates were selected by unrestricted random sampling from this pool. Free-hosted candidates were also selected randomly, but within provider strata chosen to approximate, as closely as feasible, the provider distribution observed in the phishing stratum. This matching preserves ordinary tenant pages on shared platforms while reducing provider-composition imbalance between the phishing and benign free-hosting groups.

Before inclusion, every benign candidate was screened independently with the Google Web Risk URL Lookup service \cite{googlewebrisk2026} and \secondaryvalidationservice{}. Only candidates for which neither service returned a malicious or phishing indication were retained. This dual screen reduces obvious known-threat contamination but does not establish a perfect trust universe: newly deployed, uncatalogued, or misclassified pages can still survive both checks. The resulting pool is therefore treated as a curated reference class rather than ground-truth proof of benignness.

\ifanonsubmission
Service X is the authors' own auxiliary URL-analysis service used for candidate screening.
\else
The PhiShark URL-analysis platform is an author-operated auxiliary service used for candidate screening.
\fi
Its scores and derived outputs are not included in the released evidence and are not used in the reported characterization analyses.

Benign observations were assembled as targeted source-specific snapshots rather than a continuously sampled feed. They are therefore consolidated in the source accounting, and calendar time is not used for a two-class temporal comparison against the repeatedly collected phishing feeds.

\ifanonsubmission\else
  \sourceaccountingtable
\fi

\section{Raw Artifact Preservation}

The corpus preserves the original and normalized target URL; HTTP outcomes, headers, cookies, final landing targets, and redirect chains; raw HTML and extracted text; rendered screenshots and favicons; DNS records; WHOIS/RDAP and IP WHOIS outputs; TLS certificate metadata; nameserver and mail configuration; contacted web resources; lightweight open-port observations; regional accessibility outcomes; and public compliance-path results. Screenshot capture is required for inclusion, whereas other layers retain their observed missingness.

Exact hashes are retained for transparency and reuse analysis, but they are not campaign labels.

\ifanonsubmission
  \sourceaccountingtable
\fi

\section{Hosting-Aware Evidence Model}

Free-hosted tenant pages and independently registered sites expose fundamentally different ownership boundaries. URL structure, HTML, screenshots, favicons, web retrieval, security headers, compliance paths, and TLS context remain meaningful page- or transport-level observations in both hosting strata. In contrast, DNS, WHOIS/RDAP, IP/ASN, server country, port exposure, and geo-accessibility often describe the provider when a page is hosted under a shared platform root. Prior large-scale measurements show that free website-building services are actively abused for phishing and differ operationally from self-hosted sites \cite{saharoy2022freephish,dalton2025phreshphish}. These infrastructure layers are therefore compared only in the non-free-hosting stratum.

The evidence model uses layer-specific available-case denominators. Missing fetches remain missing and are not silently recoded as negative observations. This mask prevents shared platform characteristics from being attributed to tenant pages while retaining free hosting as an operationally important part of the dataset. Table~\ref{tab:evidence-availability} reports the resulting scope and coverage.

\section{Dataset Composition and Access}
\label{sec:dataset-composition-availability}

Table~\ref{tab:source-accounting} combines source provenance, collection intervals, and the complete class-by-hosting distribution. OpenPhish contributes 30,878 scans collected between April 23 and August 15, 2026, while the Malicious Links List contributes 2,509 scans collected between June 14 and August 15, 2026. All benign reference candidates were randomly sampled from OpenPageRank; free-host selections additionally followed the provider-stratified design described above. The final corpus contains 33,387 phishing and 34,115 benign scans; 30,445 use free hosting and 37,057 use non-free hosting.

Table~\ref{tab:evidence-availability} makes the analytical denominator explicit for each layer. The lower WHOIS/RDAP and infrastructure coverage on phishing scans is itself a collection property and is kept separate from substantive class comparisons.

\begin{table*}[!t]
  \centering
  \caption{Evidence availability and hosting-aware analytical scope. Percentages use the class-level scan denominator; substantive comparisons use the layer-specific available population.}
  \label{tab:evidence-availability}
  \scriptsize
  \setlength{\tabcolsep}{3.2pt}
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{2.35cm}>{\raggedright\arraybackslash}p{2.25cm}rr>{\raggedright\arraybackslash}X}
    \toprule
    \textbf{Evidence layer} & \textbf{Analysis scope} & \textbf{Phishing availability} & \textbf{Benign availability} & \textbf{Treatment} \\
    \midrule
    Screenshot & All strata & 33,387/33,387 (100.0\%) & 34,115/34,115 (100.0\%) & Required inclusion artifact \\
    HTML & All strata & 33,099/33,387 (99.1\%) & 33,795/34,115 (99.1\%) & Page-level; available-case denominator \\
    Favicon & All strata & 23,619/33,387 (70.7\%) & 24,539/34,115 (71.9\%) & Optional artifact; missing is not negative \\
    Web fetch & All strata & 33,387/33,387 (100.0\%) & 34,115/34,115 (100.0\%) & Page-level retrieval comparison \\
    TLS & All strata & 31,853/33,387 (95.4\%) & 33,639/34,115 (98.6\%) & Transport context; hosting-stratified \\
    Security headers & All strata & 33,387/33,387 (100.0\%) & 34,115/34,115 (100.0\%) & Hosting-stratified posture \\
    Compliance paths & All strata & 32,846/33,387 (98.4\%) & 33,719/34,115 (98.8\%) & Secondary; bodies not retained \\
    DNS & Non-free only & 18,089/18,301 (98.8\%) & 18,756/18,756 (100.0\%) & Shared free-host infrastructure masked \\
    WHOIS/RDAP & Non-free only & 14,329/18,301 (78.3\%) & 17,583/18,756 (93.7\%) & Complete-case registration analysis \\
    IP geolocation & Non-free only & 14,795/18,301 (80.8\%) & 17,905/18,756 (95.5\%) & Observed hosting context only \\
    Port scan & Non-free only & 15,651/18,301 (85.5\%) & 17,905/18,756 (95.5\%) & Observed host exposure only \\
    Geo accessibility & Non-free only & 18,301/18,301 (100.0\%) & 18,756/18,756 (100.0\%) & Six-region comparison \\
    \bottomrule
  \end{tabularx}
\end{table*}

\noindent\textit{Release organization and record linkage.}
The controlled package contains a release metadata CSV and one ZIP archive per retained scan. The CSV uses \texttt{scan\_id} as a unique primary key and records the corresponding relative archive path, class and source provenance, hosting stratum, target and final-page identifiers, scan timestamps and status, and artifact-presence flags. For all 67,502 retained records, the corresponding archive is named \texttt{\string<scan\_id\string>.zip}. Table~\ref{tab:release-organization} summarizes how that identifier connects the release components.

\begin{table}[!t]
  \centering
  \caption{Controlled release organization and record linkage}
  \label{tab:release-organization}
  \scriptsize
  \setlength{\tabcolsep}{2.5pt}
  \begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{1.95cm}>{\raggedright\arraybackslash}p{1.40cm}>{\raggedright\arraybackslash}X}
    \toprule
    \textbf{Release item} & \textbf{Linkage} & \textbf{Role} \\
    \midrule
    Metadata CSV & \texttt{scan\_id} & Record index, archive path, provenance, hosting stratum, scan status, and artifact-presence flags \\
    \texttt{\string<scan\_id\string>.zip} & ZIP filename & One preserved active-web scan \\
    \texttt{metadata.json} & Archive context & Scan identity, schema, and artifact paths and hashes \\
    \texttt{data/*.json} & Archive context & Fetcher-specific observational evidence \\
    \texttt{artifacts/*} & Metadata paths & Screenshot, favicon, and losslessly compressed HTML \\
    \bottomrule
  \end{tabularx}
\end{table}

Approved researchers can first filter the release metadata CSV and obtain the unique \texttt{scan\_id} of each selected record, then open the corresponding \texttt{\string<scan\_id\string>.zip} archive. Within the archive, \texttt{metadata.json} records scan identity and artifact references, \texttt{data/*.json} contains the available fetcher-specific observations, and \texttt{artifacts/} contains the captured screenshot, favicon, and losslessly compressed HTML. Evidence extracted from different modules is joined using the enclosing scan identifier. An absent optional module or artifact is treated as unavailable evidence rather than as a negative observation.

\ifanonsubmission
Dataset documentation and an access-request interface will be made publicly available upon acceptance, while the raw corpus itself will be distributed only to approved research users. Identifying project URLs are withheld during double-blind review.
\else
Dataset documentation and its access-request interface will be publicly available through \url{https://phishark2026dataset.com} \cite{phishark2026portal}, while the raw corpus will be distributed only to approved research users.
\fi
The controlled research package covers the preserved raw evidence described above. Its release documentation will describe the metadata schema, per-scan archive layout, evidence modules, and access instructions so that approved users can inspect and analyze the provided artifacts independently.

